detrex: Benchmarking Detection Transformers

The DEtection TRansformer (DETR) algorithm has received considerable attention in the research community and is gradually emerging as a mainstream approach for object detection and other perception tasks. However, the current field lacks a unified and comprehensive benchmark specifically tailored for DETR-based models. To address this issue, we develop a unified, highly modular, and lightweight codebase called detrex, which supports a majority of the mainstream DETR-based instance recognition algorithms, covering various fundamental tasks, including object detection, segmentation, and pose estimation. We conduct extensive experiments under detrex and perform a comprehensive benchmark for DETR-based models. Moreover, we enhance the performance of detection transformers through the refinement of training hyper-parameters, providing strong baselines for supported algorithms.We hope that detrex could offer research communities a standardized and unified platform to evaluate and compare different DETR-based models while fostering a deeper understanding and driving advancements in DETR-based instance recognition. Our code is available at https://github.com/IDEA-Research/detrex. The project is currently being actively developed. We encourage the community to use detrex codebase for further development and contributions.

==> images_tex/detection_transformer_overview.tex <==
\begin{figure}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.98\linewidth]{resources/detr_design_overview.pdf}
    % \vspace{-0.1cm}
    \caption{The model design for detection transformers.\shilong{} }
    \label{fig:detr_design_overview}
    % \vspace{-0.4cm}
\end{figure}

==> images_tex/detrex_benchmark_backbone.tex <==
\begin{figure}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.98\linewidth]{resources/detrex_benchmark_backbone.pdf}
    % \vspace{-0.1cm}
    \caption{Benchmark various backbone based on DINO.
    % \shilong{list all models.} 
    }
    \label{fig:detrex_benchmark_backbone}
    % \vspace{-0.4cm}
\end{figure}

==> images_tex/detrex_design.tex <==
\begin{figure}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.98\linewidth]{resources/detrex_design.pdf}
    % \vspace{-0.1cm}
    \caption{The model design for detection transformers. 
    % \shilong{list all models.} 
    }
    \label{fig:detrex_design}
    % \vspace{-0.4cm}
\end{figure}

==> images_tex/radar_compare_detrex_and_previous_work.tex <==
\begin{figure}[h]
    \centering
    % \vspace{-0.2cm}
    \includegraphics[width=0.98\linewidth]{resources/radar_compare_detrex_and_previous_work.pdf}
    % \vspace{-0.1cm}
    \caption{Comparison of detrex implementations and previous work.}
    \label{fig:radar_compare_detrex_and_previous_work}
    % \vspace{-0.4cm}
\end{figure}

==> sec/09_insights.tex <==
\section{Analyzing Detection Transformers}
\feng{To complete. Focus on \\
1. Self-attention: classification (not limited to duplicate prediction removal\\
2. Cross-attention: box regression\\
3. Encoder: feature enhancement. Encoder dense prediction can already produce good detection performance. Its role is not so important especially when the backbone is stronger.\\
4. Decoder: iterative refine. A simple decoder-only DINO can achieve good performance.\\
5. Stack more decoder layers: need gradient to detach during training (optional).\\
6. Efficient design: decoder-only/less feature scale/interleaved encoder.\\
7. Detection performance upper bound: when manually setting all classifications as correct.
}
\subsection{Balance Classification and Box Regression}
In Decoder, self-attention is mainly responsible for classification, while cross-attention is for box regression.
\subsection{Role of Encoder and Decoder}
In DETR, the encoder is supposed to enhance image features and the decoder is to predict the detection results by querying encoder features. In advanced detectors, the encoder involves a high computational cost to produce multi-scale features but is unable to produce detection results directly. On the other side, the decoder is lightweight. To analyze the roles of encoder and decoder, we conduct experiments to with DINO~\cite{zhang2022dino}:

1. only use encoder for detection \\
2. remove the encoder and only use the decoder for detection
\feng{Maybe draw a convergence curve here of only encoder/only decoder ap curve}

Encoder dense prediction shows promising performance. Multiple decoder layers not only accelerate decoder convergence but also improves encoder convergence.

A decoder-only DINO exhibits high performance.
\subsection{Stack more Decoder Layers}
Generally, DETR-like models adopt 6 decoder layers, each of which predicts detection results and is trained with auxiliary losses. We explore the effectiveness of stacking different numbers of decoder layers.

From the experimental results, stacking more than 6 layers of the decoder can even hurt the performance of the detector. The optimization problem can be alleviated by detaching gradients in the middle.
\subsection{Efficient Design for Detection Transformer}

==> sec/checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative social impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    % \answerYes{}
    \answerNo{}
        \item Did you include complete proofs of all theoretical results?
    \answerNo{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{}
    \textcolor{orange}{We follow the common practices in the literature for model comparisons.}
\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNo{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNo{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNo{}
\end{enumerate}


\end{enumerate}

==> sec/limitations_and_borader_impact.tex <==
\section{Limitations and Broader Impact}
  

==> table_tex/benchmark_backbone_DINO_5scale.tex <==
\begin{table*}[ht]
\centering\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.5}
\footnotesize
\vspace{-0mm}
{
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l|l|l|l|cccccc|c|c|c|c|c}
\shline
Backbone & Pretrained & Feature Scales & \#epochs  & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ & \#params & GFLOPs & FPS & Memory & GPU Hours \\
\shline
R50 & ImageNet1K & 5 & 12  & $49.6$ & 67.1 & 54.2 & 32.9 & 52.4 & 63.7 & 48.0M & & & 32.9GB & 116h\\
Swin-Large & ImageNet22K & 5 & 12  & $57.5$ & 75.9 & 63.1 & 39.9 & 61.0 & 73.5 & 218.3M & & & 61.4GB & 224h \\
Swin-Large & ImageNet22K & 5 & 36  & $58.5$ & 77.0 & 64.1 & 41.4 & 62.3 & 74.0 & 218.3M & & & 61.4GB & 468h\\
Focal-Large-4level & ImageNet22K & 5 & 12  & $58.5$ & 76.8 & 64.2 & 42.2 & 62.0 & 74.1 & 228.9M & & & 67.9GB & 186h \\
ConvNeXt-Large & ImageNet22K & 5 & 12  &  &  &  &  &  &  &  & & &  &  \\
InternImage-Large & ImageNet22K & 5 & 12  &  &  &  &  &  &  &  & & &  &  \\
\shline
\end{tabular}}
\vspace{-0.2cm}
\caption{The effective of DINO-5scale based on various backbones.}
\vspace{0.2cm}
\label{tab:benchmark_backbone_on_dino_5scale}
}
\end{table*}

==> table_tex/detrex_benchmark.tex <==
\begin{table*}[ht]
\centering\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.5}
\footnotesize
\vspace{-0mm}
{
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{l|c|l|l|cccc|lll}
\shline
Model  &backbone&query type& \#epochs  & AP & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ &#params.& FLOPs &fps\\
\shline
Mask2Former & R50 &100 queries &50&43.7 &23.4& 47.2 &64.8 &44M &226G &9.7  \\
MP-Former &R50 &100 queries &50 &44.8 &24.7 &48.1& 65.5 &44M &226G &9.7 \\
Mask DINO & R50& 100 queries&50& 45.4& 25.2& 48.3& 65.8  52M &280G& 15.2\\
Mask DINO$^*$ & R50 &300 queries&50& 46.3 & 26.1& 49.3& 66.1 & 52M&286G & 14.2\\
\shline
\end{tabular}}
\vspace{-0.2cm}
\caption{The performance of segmentation transformers on COCO instance segmentation we have evaluated in our framework.}
\vspace{0.2cm}
\label{tab:comparison_detrex_with_original_implementation}
}
\end{table*}

==> table_tex/encoder_decoder.tex <==
\begin{table}[ht]
\centering\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.5}
\footnotesize
\vspace{-0mm}
{
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{c|c|c|c|ccccc}
\shline
Setting  & \#epochs & \#frozen stages & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ \\
\shline
w/o encoder  & 12  & 0 & \textbf{49.7} & 67.0 & 54.4 & 31.4 & 52.9 & 63.6  \\
DINO-4scale  & 12  & 1 & $49.4$ & 66.8 & 53.9 & 32.2 & 52.6 & 63.0  \\
DINO-4scale  & 12  & 2 & $49.4$ & 66.5 & 54.1 & 32.9 & 52.5 & 63.3 \\
\shline
DETA  & 12  & 0 & 49.8 & 67.5 & 54.7 & 31.9 & 54.2 & 65.2 \\
DETA  & 12  & 1 & \textbf{50.2} & 67.4 & 55.2 & 32.3 & 54.2 & 65.0  \\
DETA  & 12  & 2 & 49.9 & 67.3 & 54.7 & 32.1 & 54.2 & 64.8  \\
\shline
\end{tabular}}
\vspace{-0.2cm}
\caption{Ablation study on DINO and DETA with different frozen stages based on ResNet-50 backbone. The frozen stage "1" means only freezing the stem in the backbone. Frozen stage "2" means freezing the stem and the first residual stage and stage "0" means there's no frozen layer in backbone.}
\vspace{0.2cm}
\label{tab:ablation_frozen_stage}
}
\end{table}

==> table_tex/model_support.tex <==
\begin{table*}[ht]
\centering\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.2}
\footnotesize
\caption{{Supported detection transformer models of different codebases}}
\vspace{-0mm}
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{lccc}
\shline
Model & detrex & MMdetection3.0 & Detectron2 \\
\shline
DETR & \cmark  & \cmark  & \cmark \\
Deformable-DETR  & \cmark & \cmark \\
Conditional-DETR  & \cmark &  \cmark \\
Anchor-DETR & \cmark & \\
PnP-DETR  & \cmark & \\
DAB-DETR  & \cmark & \cmark \\
DAB-Deformable-DETR  & \cmark & \\
DN-DETR  & \cmark & \\
DN-Deformable-DETR  &  \cmark & \\
DINO  & \cmark &  \cmark \\
Group-DETR & \cmark & \\
$\mathcal{H}$-DETR & \cmark & \\
DETA & \cmark & \\
Stable-DINO & \cmark & \\
MaskDINO & \cmark & \\
Lite-DETR & \cmark & \\
EDPose & \cmark & \\
\shline
\end{tabular}
\label{tab:compare_with_swin_backbone}}
\end{table*}

==> table_tex/optimized_model_results.tex <==
\begin{table*}[ht]
\centering\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.5}
\footnotesize
\vspace{-3mm}
{
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c|c|c}
\shline
\multirow{2}{*}{Model}  & \multirow{2}{*}{\#epochs} & \multirow{2}{*}{Frozen stages}  & \multicolumn{3}{c|}{Learning rate} & \multirow{2}{*}{Class weight} & \multirow{2}{*}{AP}  \\ \cline{4-6}
  &  & & backbone & sampling-offsets \& reference-points & encoder-decoder &  &   \\
\shline
Deformable-DETR-Two-Stage  & 50 & 2 & 2e-5  & 2e-4 & 2e-4 & 2.0 & 46.9 \\
Deformable-DETR-Two-Stage  & 50 & 1 & 1e-5  & 1e-4 & 1e-4 & 1.0 & 48.2 \\
\shline
H-DETR  &  12 & 1  & 2e-5  & 2e-5 & 2e-4 & 2.0 & 49.1 \\
H-DETR  &  12 & 1  & 2e-5  & 2e-5 & 2e-4 & 1.0 & 48.9 \\
H-DETR  &  12 & 1  & 1e-5  & 1e-4 & 1e-4 & 2.0 & - \\
H-DETR  & 12 & 1 & 1e-5  & 1e-4 & 1e-4 & 1.0 & 48.5 \\
\shline
DETA  & 12 & 1  & 2e-5 & 2e-5 & 2e-4 & 1.0 & 50.2 \\
DETA  & 12 & 2  & 2e-5 & 2e-5 & 2e-4 & 1.0 & 49.9 \\
DETA  & 12 & 2  & 1e-5  & 1e-4 & 1e-4 & 1.0 & 49.3 \\
\shline
DINO  &  12 & 1  & 2e-5  & 2e-5 & 2e-4 & 2.0 & - \\
DINO  &  12 & 1  & 2e-5  & 2e-5 & 2e-4 & 1.0 & 49.4 \\
DINO  & 12  & 1  & 1e-5  & 1e-4 & 1e-4 & 1.0 & 49.0 \\
\shline
\end{tabular}}
\vspace{-0.2cm}
\caption{Ablation study on optimized hyper-param model for DETR variants. The frozen stage "1" means only freezing the stem in the backbone. Frozen stage "2" means freezing the stem and the first residual stage.}
\vspace{0.2cm}
\label{tab:optimized_model_results}
}
\end{table*}
